On the Necessity and Effectiveness of Learning the Prior of Variational Auto-Encoder

Using powerful posterior distributions is a popular approach to achieving better variational inference. However, recent works showed that the aggregated posterior may fail to match unit Gaussian prior, thus learning the prior becomes an alternative way to improve the lower-bound. In this paper, for the first time in the literature, we prove the necessity and effectiveness of learning the prior when aggregated posterior does not match unit Gaussian prior, analyze why this situation may happen, and propose a hypothesis that learning the prior may improve reconstruction loss, all of which are supported by our extensive experiment results. We show that using learned Real NVP prior and just one latent variable in VAE, we can achieve test NLL comparable to very deep state-of-the-art hierarchical VAE, outperforming many previous works with complex hierarchical VAE architectures.

==> metrics/dist/compare_previous/fashion_mnist_nll.tex <==

\begin{tabularx}{\linewidth}{Xr}
  \toprule
  Model & NLL \\
    \midrule
\multicolumn{2}{l}{\textit{Models without PixelCNN decoder}} \\    ConvHVAE + Lars prior$^\TwoZMark$~[\citenum{bauerResampledPriorsVariational2018}] & 225.92 \\
    \textit{Our \ConvVAE{} + RNVP $p(z)$, $K=50$} & 224.64 \\
    \textit{Our \ResnetVAE{} + RNVP $p(z)$, $K=50$} & \textbf{224.07} \\
    \midrule
\multicolumn{2}{l}{\textit{Models with PixelCNN decoder}} \\    \textit{Our \PixelVAE{} + RNVP $p(z)$, $K=50$} & \textbf{223.36} \\
  \bottomrule
\end{tabularx}
        

==> metrics/dist/compare_previous/omniglot_nll.tex <==

\begin{tabularx}{\linewidth}{Xr}
  \toprule
  Model & NLL \\
    \midrule
\multicolumn{2}{l}{\textit{Models without PixelCNN decoder}} \\    ConvHVAE + Lars prior$^\TwoZMark$~[\citenum{bauerResampledPriorsVariational2018}] & 97.08 \\
    ConvHVAE + VampPrior$^\TwoZMark$~[\citenum{tomczakVAEVampPrior2018}] & 97.56 \\
    BIVA$^\ThreeOrMoreZMark$~[\citenum{maaloeBIVAVeryDeep2019}] & \textbf{91.34} \\
    \textit{Our \ConvVAE{} + RNVP $p(z)$, $K=50$} & 93.62 \\
    \textit{Our \ResnetVAE{} + RNVP $p(z)$, $K=50$} & 93.52 \\
    \midrule
\multicolumn{2}{l}{\textit{Models with PixelCNN decoder}} \\    VLAE$^\ThreeOrMoreZMark$~[\citenum{chenVariationalLossyAutoencoder2016}] & 89.83 \\
    PixelHVAE + VampPrior$^\TwoZMark$~[\citenum{tomczakVAEVampPrior2018}] & 89.76 \\
    \textit{Our \PixelVAE{} + RNVP $p(z)$, $K=50$} & \textbf{89.60} \\
  \bottomrule
\end{tabularx}
        

==> metrics/dist/dual_rnvp/recons_mean_only.tex <==

\begin{tabular}{cccc}
  \toprule
  & \multicolumn{3}{c}{\tablehr{\ResnetVAE}} \\
  \cmidrule(lr){2-4}
  \tablehr{Datasets}  & \parbox[c]{3em}{RNVP \\ \centering \(q(z|x)\)}  & \parbox[c]{3em}{RNVP \\ \centering \(p(z)\)}  & both  \\
  \midrule
    \StaticMNIST{} 
 &
-58.10 &
\textbf{-54.32} &
-54.99    \\
    \MNIST{} 
 &
-56.15 &
\textbf{-53.64} &
-53.76    \\
    \FashionMNIST{} 
 &
-206.61 &
\textbf{-204.66} &
-204.76    \\
    \Omniglot{} 
 &
-63.34 &
\textbf{-61.21} &
-61.88    \\
  \bottomrule
\end{tabular}
        

==> metrics/dist/dual_rnvp/recons_with_std.tex <==

\begin{tabular}{cccc}
  \toprule
  & \multicolumn{3}{c}{\tablehr{\ResnetVAE}} \\
  \cmidrule(lr){2-4}
  \tablehr{Datasets}  & \parbox[c]{3em}{RNVP \\ \centering \(q(z|x)\)}  & \parbox[c]{3em}{RNVP \\ \centering \(p(z)\)}  & both  \\
  \midrule
    \StaticMNIST{} 
 &
-58.10 $\pm$ 0.16 &
\textbf{-54.32 $\pm$ 0.09} &
-54.99 $\pm$ 0.32    \\
    \MNIST{} 
 &
-56.15 $\pm$ 0.06 &
\textbf{-53.64 $\pm$ 0.03} &
-53.76 $\pm$ 0.03    \\
    \FashionMNIST{} 
 &
-206.61 $\pm$ 0.01 &
\textbf{-204.66 $\pm$ 0.05} &
-204.76 $\pm$ 0.03    \\
    \Omniglot{} 
 &
-63.34 $\pm$ 0.03 &
\textbf{-61.21 $\pm$ 0.07} &
-61.88 $\pm$ 0.06    \\
  \bottomrule
\end{tabular}
        

==> metrics/dist/flow_layer_tests/recons_mean_only.tex <==

\begin{tabular}{ccccccccc}
  \toprule
  & \multicolumn{8}{c}{\tablehr{Flow depth $K$ for \RealNVP{} prior}} \\
  \cmidrule(lr){2-9}
  \tablehr{Datasets}  & 0  & 1  & 2  & 5  & 10  & 20  & 30  & 50  \\
  \midrule
    \StaticMNIST{}
      & -60.09      & -57.67      & -56.86      & -55.89      & -54.98      & -54.32      & -54.02      & \textbf{-53.48}    \\
    \MNIST{}
      & -58.70      & -56.45      & -55.75      & -54.70      & -54.00      & -53.64      & -53.53      & \textbf{-53.44}    \\
    \FashionMNIST{}
      & -208.94      & -207.02      & -206.17      & -205.18      & -204.80      & -204.66      & -204.61      & \textbf{-204.59}    \\
    \Omniglot{}
      & -66.98      & -66.56      & -65.15      & -63.54      & -62.15      & -61.21      & \textbf{-60.94}      & -60.96    \\
  \bottomrule
\end{tabular}
        

==> metrics/dist/flow_layer_tests/recons_with_std.tex <==

\begin{tabular}{ccccc}
  \toprule
  & \multicolumn{4}{c}{\tablehr{Datasets}} \\
  \cmidrule(lr){2-5}
  \tablehr{Flow depth}  & \StaticMNIST{}  & \MNIST{}  & \FashionMNIST{}  & \Omniglot{}  \\
  \midrule
    0 
 &
-60.09 $\pm$ 0.20 &
-58.70 $\pm$ 0.09 &
-208.94 $\pm$ 0.08 &
-66.98 $\pm$ 0.20    \\
    1 
 &
-57.67 $\pm$ 0.42 &
-56.45 $\pm$ 0.03 &
-207.02 $\pm$ 0.04 &
-66.56 $\pm$ 0.20    \\
    2 
 &
-56.86 $\pm$ 0.06 &
-55.75 $\pm$ 0.05 &
-206.17 $\pm$ 0.06 &
-65.15 $\pm$ 0.15    \\
    5 
 &
-55.89 $\pm$ 0.05 &
-54.70 $\pm$ 0.05 &
-205.18 $\pm$ 0.03 &
-63.54 $\pm$ 0.16    \\
    10 
 &
-54.98 $\pm$ 0.23 &
-54.00 $\pm$ 0.04 &
-204.80 $\pm$ 0.03 &
-62.15 $\pm$ 0.14    \\
    20 
 &
-54.32 $\pm$ 0.09 &
-53.64 $\pm$ 0.03 &
-204.66 $\pm$ 0.05 &
-61.21 $\pm$ 0.07    \\
    30 
 &
-54.02 $\pm$ 0.06 &
-53.53 $\pm$ 0.05 &
-204.61 $\pm$ 0.04 &
\textbf{-60.94 $\pm$ 0.03}    \\
    50 
 &
\textbf{-53.48 $\pm$ 0.13} &
\textbf{-53.44 $\pm$ 0.05} &
\textbf{-204.59 $\pm$ 0.02} &
-60.96 $\pm$ 0.06    \\
  \bottomrule
\end{tabular}
        

==> metrics/dist/kl_recons/ConvVAE.tex <==

    \begin{tabular}{ccccccccc}
    \toprule
& \multicolumn{4}{c}{\tablehr{standard}}& \multicolumn{4}{c}{\tablehr{RNVP \(p(z)\)}} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}    \tablehr{Datasets} & \textit{lb}& \textit{recons}& \textit{kl}& $kl_{z|x}$ & \textit{lb}& \textit{recons}& \textit{kl}& $kl_{z|x}$ \\
    \midrule
        \StaticMNIST{}
 & 
-88.15 & 
-60.34 & 
\textbf{27.81} & 
4.51 & 
\textbf{-82.91} & 
\textbf{-54.01} & 
28.90 & 
\textbf{2.86}        \\
        \MNIST{}
 & 
-85.89 & 
-58.97 & 
\textbf{26.92} & 
3.75 & 
\textbf{-80.42} & 
\textbf{-53.33} & 
27.09 & 
\textbf{1.75}        \\
        \FashionMNIST{}
 & 
-230.43 & 
-210.24 & 
\textbf{20.18} & 
2.92 & 
\textbf{-226.65} & 
\textbf{-204.93} & 
21.72 & 
\textbf{2.00}        \\
        \Omniglot{}
 & 
-104.70 & 
-66.00 & 
\textbf{38.70} & 
6.83 & 
\textbf{-98.59} & 
\textbf{-59.07} & 
39.51 & 
\textbf{4.91}        \\
    \bottomrule
    \end{tabular}
            

==> metrics/dist/kl_recons/DenseVAE.tex <==

    \begin{tabular}{ccccccccc}
    \toprule
& \multicolumn{4}{c}{\tablehr{standard}}& \multicolumn{4}{c}{\tablehr{RNVP \(p(z)\)}} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}    \tablehr{Datasets} & \textit{lb}& \textit{recons}& \textit{kl}& $kl_{z|x}$ & \textit{lb}& \textit{recons}& \textit{kl}& $kl_{z|x}$ \\
    \midrule
        \StaticMNIST{}
 & 
-94.53 & 
-65.54 & 
29.00 & 
5.69 & 
\textbf{-88.87} & 
\textbf{-63.35} & 
\textbf{25.52} & 
\textbf{4.00}        \\
        \MNIST{}
 & 
-88.19 & 
-62.04 & 
\textbf{26.16} & 
3.71 & 
\textbf{-82.57} & 
\textbf{-55.99} & 
26.58 & 
\textbf{2.14}        \\
        \FashionMNIST{}
 & 
-230.81 & 
-211.71 & 
\textbf{19.11} & 
2.22 & 
\textbf{-227.72} & 
\textbf{-208.13} & 
19.59 & 
\textbf{1.61}        \\
        \Omniglot{}
 & 
-113.59 & 
-78.25 & 
35.33 & 
7.17 & 
\textbf{-107.99} & 
\textbf{-73.10} & 
\textbf{34.89} & 
\textbf{5.80}        \\
    \bottomrule
    \end{tabular}
            

==> metrics/dist/kl_recons/PixelVAE.tex <==

    \begin{tabular}{ccccccccc}
    \toprule
& \multicolumn{4}{c}{\tablehr{standard}}& \multicolumn{4}{c}{\tablehr{RNVP \(p(z)\)}} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}    \tablehr{Datasets} & \textit{lb}& \textit{recons}& \textit{kl}& $kl_{z|x}$ & \textit{lb}& \textit{recons}& \textit{kl}& $kl_{z|x}$ \\
    \midrule
        \StaticMNIST{}
 & 
-81.06 & 
-69.02 & 
\textbf{12.03} & 
\textbf{1.59} & 
\textbf{-80.60} & 
\textbf{-62.22} & 
18.38 & 
1.68        \\
        \MNIST{}
 & 
-79.88 & 
-68.73 & 
\textbf{11.15} & 
1.24 & 
\textbf{-79.28} & 
\textbf{-64.41} & 
14.87 & 
\textbf{1.13}        \\
        \FashionMNIST{}
 & 
-225.60 & 
-214.15 & 
\textbf{11.45} & 
1.38 & 
\textbf{-224.65} & 
\textbf{-210.16} & 
14.49 & 
\textbf{1.26}        \\
        \Omniglot{}
 & 
\textbf{-91.58} & 
-82.80 & 
\textbf{8.78} & 
\textbf{1.75} & 
-91.78 & 
\textbf{-79.70} & 
12.07 & 
2.16        \\
    \bottomrule
    \end{tabular}
            

==> metrics/dist/kl_recons_2/kl_recons_ConvVAE.tex <==

\begin{tabular}{ccccc}
\toprule
& \multicolumn{4}{c}{\tablehr{standard}} \\
\cmidrule(lr){2-5}\tablehr{Datasets} & \textit{elbo}& \textit{recons}& \textit{kl}& $kl_{z|x}$ \\
\midrule
    \StaticMNIST{}
 & 
-88.15 & 
-60.34 & 
27.81 & 
4.51    \\
    \MNIST{}
 & 
-85.89 & 
-58.97 & 
26.92 & 
3.75    \\
    \FashionMNIST{}
 & 
-230.43 & 
-210.24 & 
\textbf{20.18} & 
2.92    \\
    \Omniglot{}
 & 
-104.70 & 
-66.00 & 
38.70 & 
6.83    \\
            

\midrule
& \multicolumn{4}{c}{\tablehr{RNVP \(q(z|x)\)}} \\
\cmidrule(lr){2-5}\tablehr{Datasets} & \textit{elbo}& \textit{recons}& \textit{kl}& $kl_{z|x}$ \\
\midrule
    \StaticMNIST{}
 & 
-83.92 & 
-56.67 & 
\textbf{27.25} & 
\textbf{2.82}    \\
    \MNIST{}
 & 
-82.46 & 
-56.08 & 
\textbf{26.38} & 
2.37    \\
    \FashionMNIST{}
 & 
-228.20 & 
-207.33 & 
20.88 & 
2.18    \\
    \Omniglot{}
 & 
-99.92 & 
-62.48 & 
\textbf{37.44} & 
5.02    \\
            

\midrule
& \multicolumn{4}{c}{\tablehr{RNVP \(p(z)\)}} \\
\cmidrule(lr){2-5}\tablehr{Datasets} & \textit{elbo}& \textit{recons}& \textit{kl}& $kl_{z|x}$ \\
\midrule
    \StaticMNIST{}
 & 
\textbf{-82.91} & 
\textbf{-54.01} & 
28.90 & 
2.86    \\
    \MNIST{}
 & 
\textbf{-80.42} & 
\textbf{-53.33} & 
27.09 & 
\textbf{1.75}    \\
    \FashionMNIST{}
 & 
\textbf{-226.65} & 
\textbf{-204.93} & 
21.72 & 
\textbf{2.00}    \\
    \Omniglot{}
 & 
\textbf{-98.59} & 
\textbf{-59.07} & 
39.51 & 
\textbf{4.91}    \\
\bottomrule
\end{tabular}
            

==> metrics/dist/kl_recons_2/kl_recons_DenseVAE.tex <==

\begin{tabular}{ccccc}
\toprule
& \multicolumn{4}{c}{\tablehr{standard}} \\
\cmidrule(lr){2-5}\tablehr{Datasets} & \textit{elbo}& \textit{recons}& \textit{kl}& $kl_{z|x}$ \\
\midrule
    \StaticMNIST{}
 & 
-94.53 & 
-65.54 & 
29.00 & 
5.69    \\
    \MNIST{}
 & 
-88.19 & 
-62.04 & 
\textbf{26.16} & 
3.71    \\
    \FashionMNIST{}
 & 
-230.81 & 
-211.71 & 
\textbf{19.11} & 
2.22    \\
    \Omniglot{}
 & 
-113.59 & 
-78.25 & 
35.33 & 
7.17    \\
            

\midrule
& \multicolumn{4}{c}{\tablehr{RNVP \(q(z|x)\)}} \\
\cmidrule(lr){2-5}\tablehr{Datasets} & \textit{elbo}& \textit{recons}& \textit{kl}& $kl_{z|x}$ \\
\midrule
    \StaticMNIST{}
 & 
-90.78 & 
\textbf{-62.55} & 
28.23 & 
4.71    \\
    \MNIST{}
 & 
-85.15 & 
-58.83 & 
26.31 & 
2.62    \\
    \FashionMNIST{}
 & 
-229.53 & 
-210.35 & 
19.18 & 
1.75    \\
    \Omniglot{}
 & 
-108.54 & 
-73.71 & 
\textbf{34.83} & 
\textbf{5.57}    \\
            

\midrule
& \multicolumn{4}{c}{\tablehr{RNVP \(p(z)\)}} \\
\cmidrule(lr){2-5}\tablehr{Datasets} & \textit{elbo}& \textit{recons}& \textit{kl}& $kl_{z|x}$ \\
\midrule
    \StaticMNIST{}
 & 
\textbf{-88.87} & 
-63.35 & 
\textbf{25.52} & 
\textbf{4.00}    \\
    \MNIST{}
 & 
\textbf{-82.57} & 
\textbf{-55.99} & 
26.58 & 
\textbf{2.14}    \\
    \FashionMNIST{}
 & 
\textbf{-227.72} & 
\textbf{-208.13} & 
19.59 & 
\textbf{1.61}    \\
    \Omniglot{}
 & 
\textbf{-107.99} & 
\textbf{-73.10} & 
34.89 & 
5.80    \\
\bottomrule
\end{tabular}
            

==> metrics/dist/kl_recons_2/kl_recons_PixelVAE.tex <==

\begin{tabular}{ccccc}
\toprule
& \multicolumn{4}{c}{\tablehr{standard}} \\
\cmidrule(lr){2-5}\tablehr{Datasets} & \textit{elbo}& \textit{recons}& \textit{kl}& $kl_{z|x}$ \\
\midrule
    \StaticMNIST{}
 & 
-81.06 & 
-69.02 & 
\textbf{12.03} & 
1.59    \\
    \MNIST{}
 & 
-79.88 & 
-68.73 & 
\textbf{11.15} & 
1.24    \\
    \FashionMNIST{}
 & 
-225.60 & 
-214.15 & 
\textbf{11.45} & 
1.38    \\
    \Omniglot{}
 & 
-91.58 & 
-82.80 & 
8.78 & 
1.75    \\
            

\midrule
& \multicolumn{4}{c}{\tablehr{RNVP \(q(z|x)\)}} \\
\cmidrule(lr){2-5}\tablehr{Datasets} & \textit{elbo}& \textit{recons}& \textit{kl}& $kl_{z|x}$ \\
\midrule
    \StaticMNIST{}
 & 
-80.65 & 
-67.91 & 
12.75 & 
\textbf{1.57}    \\
    \MNIST{}
 & 
-79.59 & 
-68.17 & 
11.42 & 
1.18    \\
    \FashionMNIST{}
 & 
-225.05 & 
-213.41 & 
11.64 & 
\textbf{1.24}    \\
    \Omniglot{}
 & 
\textbf{-91.26} & 
-83.17 & 
\textbf{8.10} & 
\textbf{1.57}    \\
            

\midrule
& \multicolumn{4}{c}{\tablehr{RNVP \(p(z)\)}} \\
\cmidrule(lr){2-5}\tablehr{Datasets} & \textit{elbo}& \textit{recons}& \textit{kl}& $kl_{z|x}$ \\
\midrule
    \StaticMNIST{}
 & 
\textbf{-80.60} & 
\textbf{-62.22} & 
18.38 & 
1.68    \\
    \MNIST{}
 & 
\textbf{-79.28} & 
\textbf{-64.41} & 
14.87 & 
\textbf{1.13}    \\
    \FashionMNIST{}
 & 
\textbf{-224.65} & 
\textbf{-210.16} & 
14.49 & 
1.26    \\
    \Omniglot{}
 & 
-91.78 & 
\textbf{-79.70} & 
12.07 & 
2.16    \\
\bottomrule
\end{tabular}
            

==> metrics/dist/kl_recons_2/kl_recons_ResnetVAE.tex <==

\begin{tabular}{ccccc}
\toprule
& \multicolumn{4}{c}{\tablehr{standard}} \\
\cmidrule(lr){2-5}\tablehr{Datasets} & \textit{elbo}& \textit{recons}& \textit{kl}& $kl_{z|x}$ \\
\midrule
    \StaticMNIST{}
 & 
-87.61 & 
-60.09 & 
27.52 & 
4.67    \\
    \MNIST{}
 & 
-84.62 & 
-58.70 & 
25.92 & 
3.55    \\
    \FashionMNIST{}
 & 
-228.91 & 
-208.94 & 
\textbf{19.96} & 
2.74    \\
    \Omniglot{}
 & 
-104.87 & 
-66.98 & 
37.89 & 
7.88    \\
            

\midrule
& \multicolumn{4}{c}{\tablehr{RNVP \(q(z|x)\)}} \\
\cmidrule(lr){2-5}\tablehr{Datasets} & \textit{elbo}& \textit{recons}& \textit{kl}& $kl_{z|x}$ \\
\midrule
    \StaticMNIST{}
 & 
-84.72 & 
-58.10 & 
\textbf{26.63} & 
3.75    \\
    \MNIST{}
 & 
-81.95 & 
-56.15 & 
\textbf{25.80} & 
2.42    \\
    \FashionMNIST{}
 & 
-227.16 & 
-206.61 & 
20.54 & 
2.14    \\
    \Omniglot{}
 & 
-100.30 & 
-63.34 & 
\textbf{36.96} & 
6.00    \\
            

\midrule
& \multicolumn{4}{c}{\tablehr{RNVP \(p(z)\)}} \\
\cmidrule(lr){2-5}\tablehr{Datasets} & \textit{elbo}& \textit{recons}& \textit{kl}& $kl_{z|x}$ \\
\midrule
    \StaticMNIST{}
 & 
\textbf{-82.85} & 
\textbf{-54.32} & 
28.54 & 
\textbf{2.87}    \\
    \MNIST{}
 & 
\textbf{-80.34} & 
\textbf{-53.64} & 
26.70 & 
\textbf{1.76}    \\
    \FashionMNIST{}
 & 
\textbf{-225.97} & 
\textbf{-204.66} & 
21.31 & 
\textbf{1.88}    \\
    \Omniglot{}
 & 
\textbf{-99.60} & 
\textbf{-61.21} & 
38.39 & 
\textbf{5.99}    \\
\bottomrule
\end{tabular}
            

==> metrics/dist/main_experiments/recons_mean_only.tex <==

\begin{tabular}{cccccccccc}
  \toprule & \multicolumn{3}{c}{\tablehr{\DenseVAE{}}}  & \multicolumn{3}{c}{\tablehr{\ResnetVAE{}}}  & \multicolumn{3}{c}{\tablehr{\PixelVAE{}}}  \\
 \cmidrule(lr){2-4}  \cmidrule(lr){5-7}  \cmidrule(lr){8-10}   \tablehr{Datasets} & standard & \parbox[c]{3em}{\centering RNVP \\ \(q(z|x)\)} & \parbox[c]{3em}{\centering RNVP \\ \(p(z)\)} & standard & \parbox[c]{3em}{\centering RNVP \\ \(q(z|x)\)} & \parbox[c]{3em}{\centering RNVP \\ \(p(z)\)} & standard & \parbox[c]{3em}{\centering RNVP \\ \(q(z|x)\)} & \parbox[c]{3em}{\centering RNVP \\ \(p(z)\)} \\
  \midrule
    \StaticMNIST{}
 &
-65.54 &
\textbf{-62.55} &
-63.35 &
-60.09 &
-58.10 &
\textbf{-54.32} &
-69.02 &
-67.91 &
\textbf{-62.22}    \\
    \MNIST{}
 &
-62.04 &
-58.83 &
\textbf{-55.99} &
-58.70 &
-56.15 &
\textbf{-53.64} &
-68.73 &
-68.17 &
\textbf{-64.41}    \\
    \FashionMNIST{}
 &
-211.71 &
-210.35 &
\textbf{-208.13} &
-208.94 &
-206.61 &
\textbf{-204.66} &
-214.15 &
-213.41 &
\textbf{-210.16}    \\
    \Omniglot{}
 &
-78.25 &
-73.71 &
\textbf{-73.10} &
-66.98 &
-63.34 &
\textbf{-61.21} &
-82.80 &
-83.17 &
\textbf{-79.70}    \\
\bottomrule
\end{tabular}        

==> metrics/dist/main_experiments/recons_with_std.tex <==

\begin{tabular}{cccccc}
  \toprule
  & & \multicolumn{4}{c}{\tablehr{Datasets}} \\
  \cmidrule(lr){3-6}
  \multicolumn{2}{c}{\tablehr{Models}}  & \StaticMNIST{}  & \MNIST{}  & \FashionMNIST{}  & \Omniglot{}  \\
  \midrule
    \multirow{3}{*}{\DenseVAE{}} &
      standard 
 &
-65.54 $\pm$ 0.14 &
-62.04 $\pm$ 0.03 &
-211.71 $\pm$ 0.10 &
-78.25 $\pm$ 0.15      \\
 &       RNVP \(q(z|x)\) 
 &
\textbf{-62.55 $\pm$ 0.46} &
-58.83 $\pm$ 0.04 &
-210.35 $\pm$ 0.04 &
-73.71 $\pm$ 0.16      \\
 &       RNVP \(p(z)\) 
 &
-63.35 $\pm$ 0.03 &
\textbf{-55.99 $\pm$ 0.02} &
\textbf{-208.13 $\pm$ 0.06} &
\textbf{-73.10 $\pm$ 0.28}      \\
\cmidrule(lr){1-6}    \multirow{3}{*}{\ConvVAE{}} &
      standard 
 &
-60.34 $\pm$ 0.11 &
-58.97 $\pm$ 0.02 &
-210.24 $\pm$ 0.08 &
-66.00 $\pm$ 0.18      \\
 &       RNVP \(q(z|x)\) 
 &
-56.67 $\pm$ 0.12 &
-56.08 $\pm$ 0.03 &
-207.33 $\pm$ 0.09 &
-62.48 $\pm$ 0.17      \\
 &       RNVP \(p(z)\) 
 &
\textbf{-54.01 $\pm$ 0.24} &
\textbf{-53.33 $\pm$ 0.03} &
\textbf{-204.93 $\pm$ 0.03} &
\textbf{-59.07 $\pm$ 0.03}      \\
\cmidrule(lr){1-6}    \multirow{3}{*}{\ResnetVAE{}} &
      standard 
 &
-60.09 $\pm$ 0.20 &
-58.70 $\pm$ 0.09 &
-208.94 $\pm$ 0.08 &
-66.98 $\pm$ 0.20      \\
 &       RNVP \(q(z|x)\) 
 &
-58.10 $\pm$ 0.16 &
-56.15 $\pm$ 0.06 &
-206.61 $\pm$ 0.01 &
-63.34 $\pm$ 0.03      \\
 &       RNVP \(p(z)\) 
 &
\textbf{-54.32 $\pm$ 0.09} &
\textbf{-53.64 $\pm$ 0.03} &
\textbf{-204.66 $\pm$ 0.05} &
\textbf{-61.21 $\pm$ 0.07}      \\
\cmidrule(lr){1-6}    \multirow{3}{*}{\PixelVAE{}} &
      standard 
 &
-69.02 $\pm$ 0.01 &
-68.73 $\pm$ 0.16 &
-214.15 $\pm$ 0.10 &
-82.80 $\pm$ 0.23      \\
 &       RNVP \(q(z|x)\) 
 &
-67.91 $\pm$ 0.07 &
-68.17 $\pm$ 0.07 &
-213.41 $\pm$ 0.06 &
-83.17 $\pm$ 0.31      \\
 &       RNVP \(p(z)\) 
 &
\textbf{-62.22 $\pm$ 0.10} &
\textbf{-64.41 $\pm$ 0.41} &
\textbf{-210.16 $\pm$ 0.26} &
\textbf{-79.70 $\pm$ 0.09}      \\
  \bottomrule
\end{tabular}
        

==> metrics/dist/post_train/recons_mean_only.tex <==

\begin{tabular}{ccccc}
  \toprule
  & \multicolumn{4}{c}{\tablehr{\ResnetVAE}} \\
  \cmidrule(lr){2-5}
  \tablehr{Datasets}  & joint  & iterative  & post-hoc  & none  \\
  \midrule
    \StaticMNIST{} 
 &
\textbf{-54.32} &
-57.97 &
-60.10 &
-60.09    \\
    \MNIST{} 
 &
\textbf{-53.64} &
-57.15 &
-58.70 &
-58.70    \\
    \FashionMNIST{} 
 &
\textbf{-204.66} &
-207.83 &
-208.94 &
-208.94    \\
    \Omniglot{} 
 &
\textbf{-61.21} &
-63.28 &
-66.98 &
-66.98    \\
  \bottomrule
\end{tabular}
        

==> metrics/dist/post_train/recons_with_std.tex <==

\begin{tabular}{ccccc}
  \toprule
  & \multicolumn{4}{c}{\tablehr{\ResnetVAE}} \\
  \cmidrule(lr){2-5}
  \tablehr{Datasets}  & joint  & iterative  & post-hoc  & none  \\
  \midrule
    \StaticMNIST{} 
 &
\textbf{-54.32 $\pm$ 0.09} &
-57.97 $\pm$ 0.18 &
-60.10 $\pm$ 0.20 &
-60.09 $\pm$ 0.20    \\
    \MNIST{} 
 &
\textbf{-53.64 $\pm$ 0.03} &
-57.15 $\pm$ 0.08 &
-58.70 $\pm$ 0.09 &
-58.70 $\pm$ 0.09    \\
    \FashionMNIST{} 
 &
\textbf{-204.66 $\pm$ 0.05} &
-207.83 $\pm$ 0.05 &
-208.94 $\pm$ 0.08 &
-208.94 $\pm$ 0.08    \\
    \Omniglot{} 
 &
\textbf{-61.21 $\pm$ 0.07} &
-63.28 $\pm$ 0.25 &
-66.98 $\pm$ 0.20 &
-66.98 $\pm$ 0.20    \\
  \bottomrule
\end{tabular}
        
